Understanding and Exploiting Design-Induced Latency Variation in Modern DRAM Chips

Variation has been shown to exist across the cells within a modern DRAM chip. We empirically demonstrate a new form of variation that exists within a real DRAM chip, induced by the design and placement of different components in the DRAM chip. Our goals are to understand design-induced variation that exists in real, state-of-the-art DRAM chips, exploit it to develop low-cost mechanisms that can dynamically find and use the lowest latency at which to operate a DRAM chip reliably, and, thus, improve overall system performance while ensuring reliable system operation. To this end, we first experimentally demonstrate and analyze designed-induced variation in modern DRAM devices by testing and characterizing 96 DIMMs (768 DRAM chips). Our characterization identifies DRAM regions that are vulnerable to errors, if operated at lower latency, and finds consistency in their locations across a given DRAM chip generation, due to design-induced variation. Based on our extensive experimental analysis, we develop two mechanisms that reliably reduce DRAM latency. First, DIVA Profiling uses runtime profiling to dynamically identify the lowest DRAM latency that does not introduce failures. DIVA Profiling exploits design-induced variation and periodically profiles only the vulnerable regions to determine the lowest DRAM latency at low cost. Our second mechanism, DIVA Shuffling, shuffles data such that values stored in vulnerable regions are mapped to multiple error-correcting code (ECC) codewords. Combined together, our two mechanisms reduce read/write latency by 40.0%/60.5%, which translates to an overall system performance improvement of 14.7%/13.7%/13.8% (in 2-/4-/8-core systems) across a variety of workloads, while ensuring reliable operation.

==> fig/mech_lowlatency.tex <==
\begin{figure}[h]
	\vspace{-0.05in}
	\centering
	\includegraphics[width=0.7\linewidth]{fig/pdf/mech_lowlatency}
	\vspace{-0.05in}
	\caption{Design-Induced Variation Aware Online Profiling}
	\label{fig:mech_lowlatency}
	\vspace{-0.05in}
\end{figure}


==> fig/profile_timings.tex <==
\begin{figure}[h]
	\vspace{-0.05in}
	\centering
	\subfloat[\trcd] {
		\includegraphics[height=1.5in]{fig/pdf/profile_trcd}
		\label{fig:profile_trcd}
	}
	\subfloat[\tras] {
		\includegraphics[height=1.5in]{fig/pdf/profile_tras}
		\label{fig:profile_tras}
	}

	\vspace{-0.05in}
	\subfloat[\trp] {
		\includegraphics[height=1.5in]{fig/pdf/profile_trp}
		\label{fig:profile_trp}
	}
	\subfloat[\twr] {
		\includegraphics[height=1.5in]{fig/pdf/profile_twr}
		\label{fig:profile_twr}
	}
	\vspace{-0.05in}
	\caption{Latency Reduction for each Timing Parameter}
	\label{fig:profile_timings}
	\vspace{-0.05in}
\end{figure}


==> fig/sim_model.tex <==
\begin{figure}[h]
	\vspace{-0.10in}
	\centering
	\includegraphics[height=2in]{fig/pdf/sim_model}
	\vspace{-0.10in}
	\caption{A Detailed Mat Model That Including Parasitic Resistance and Capacitance}
	\label{fig:sim_model}
	\vspace{-0.10in}
\end{figure}



==> fig/simulation.tex <==
\begin{figure}[h]
	\vspace{0.10in}
	\centering
	\subfloat[Design-Induced Variation in Bitline] {
		\includegraphics[height=3in]{fig/pdf/sim_bitline}
		\label{fig:sim_bitline}
	}
	\vspace{-0.1in}

	\subfloat[Design-Induced Variation in Wordline] {
		\includegraphics[height=3in]{fig/pdf/sim_wordline}
		\label{fig:sim_wordline}
	}
	\vspace{-0.05in}
	\caption{Simulation Results of Design-Induced Variation}
	\label{fig:simulation}
	\vspace{-0.15in}
\end{figure}



==> sec/abstract_upload.tex <==
Variation has been shown to exist across the cells within a modern DRAM chip.
Prior work has studied and exploited several forms of variation, such as
manufacturing-process- or temperature-induced variation. We empirically
demonstrate a new form of variation that exists within a real DRAM chip, induced
by the design and placement of different components in the DRAM chip: different
regions in DRAM, based on their relative distances from the peripheral
structures, require different minimum access latencies for reliable operation.
In particular, we show that in most real DRAM chips, cells closer to the
peripheral structures can be accessed much faster than cells that are farther.
We call this phenomenon design-induced variation in DRAM. Our goals are to i)
understand design-induced variation that exists in real, state-of-the-art DRAM
chips, ii) exploit it to develop low-cost mechanisms that can dynamically find
and use the lowest latency at which to operate a DRAM chip reliably, and, thus,
iii) improve overall system performance while ensuring reliable system
operation.

To this end, we first experimentally demonstrate and analyze designed-induced
variation in modern DRAM devices by testing and characterizing 96 DIMMs (768
DRAM chips). Our characterization identifies DRAM regions that are vulnerable to
errors, if operated at lower latency, and finds consistency in their locations
across a given DRAM chip generation, due to design-induced variation. Based on
our extensive experimental analysis, we develop two mechanisms that reliably
reduce DRAM latency. First, DIVA Profiling uses runtime profiling to dynamically
identify the lowest DRAM latency that does not introduce failures. DIVA
Profiling exploits design-induced variation and periodically profiles only the
vulnerable regions to determine the lowest DRAM latency at low cost. It is the
first mechanism to dynamically determine the lowest latency that can be used to
operate DRAM reliably. DIVA Profiling reduces the latency of read/write requests
by 35.1%/57.8%, respectively, at 55C. Our second mechanism, DIVA Shuffling,
shuffles data such that values stored in vulnerable regions are mapped to
multiple error-correcting code (ECC) codewords. As a result, DIVA Shuffling can
correct 26% more multi-bit errors than conventional ECC. Combined together, our
two mechanisms reduce read/write latency by 40.0%/60.5%, which translates to an
overall system performance improvement of 14.7%/13.7%/13.8% (in 2-/4-/8-core
systems) across a variety of workloads, while ensuring reliable operation.


==> tbl/repo/modules.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[h]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Design-Induced Variation$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} 

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize tRC (ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize Die Version$^{\S}$} 
 & {\em \footnotesize tRP} 
 & {\em \footnotesize tRCD} \\

\midrule

%% HYNIX
\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\cellcolor{white} & \module{A}{11}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{12}{} & 11-31 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 4.3  & --	  \\
\cellcolor{white} & \module{A}{13}{} & 11-42 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 4.9  & 93.7 \\
\cellcolor{white} & \module{A}{14}{} & 12-08 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 96.7 & 28.6 \\
\cellcolor{white} & \module{A}{15}{} & 12-12 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 3.9  & 45.2 \\
\cellcolor{white} & \module{A}{16}{} & 12-12 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 103  & 373  \\
\cellcolor{white} & \module{A}{17}{} & 12-20 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 31.4 & 178  \\
\cellcolor{white} & \module{A}{18}{} & 12-20 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{19}{} & 12-24 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 37.1 & 21.3 \\
\cellcolor{white} & \module{A}{20}{} & 12-26 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 26.7 & 26.9 \\
\cellcolor{white} & \module{A}{21}{} & 12-32 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 61.3 & 160  \\
\cellcolor{white} & \module{A}{22}{} & 12-37 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 9.9  & 44.3 \\
\cellcolor{white} & \module{A}{23}{} & 12-37 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 161  & 37.1 \\
\cellcolor{white} & \module{A}{24}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 54.4 & 196  \\
\cellcolor{white} & \module{A}{25}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 24.1 & 1034 \\
\cellcolor{white} & \module{A}{26}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 208  & 55.8 \\
\cellcolor{white} & \module{A}{27}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 88.3 & 20.8 \\
\cellcolor{white} & \module{A}{28}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 51.6 & 122  \\
\cellcolor{white} & \module{A}{29}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 31.8 & 100  \\
\multirow{-32}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\bottomrule

\end{tabular}

\begin{tabular}{lp{10cm}}

{$\,$} \\

{\footnotesize $\ast$ We report the manufacturing date in a year-week (yy-ww)
format. For example, 15-01 means that the DIMM was manufactured during} \\
{\hspace{0.1in}the first week of 2015.} \\ 

{$\,$} \\

{\footnotesize $\ddagger$ The maximum DRAM chip size supported by our testing
platform is 2Gb.} \\

{$\,$} \\

{\footnotesize $\S$ We report the DRAM die versions that are marked on the chip package.
Since the die version changes when the DRAM design changes,}\\
{\hspace{0.1in}we expect and observe that DIMMs with the same die version have similar
design-induced variation.} \\

{$\,$} \\

{\footnotesize $\star$ We report the {\em vulnerability ratio}, which we
define as the ratio of the number errors that occur the top 10\% of the most vulnerable and}\\
{\hspace{0.1in}least vulnerable rows, to show design-induced variation in timing parameters.}
\\

\end{tabular}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em A} (sorted by manufacturing date)} 
\label{tbl:vendor1}

\end{table*}




\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Design-Induced Variation$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} 

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize tRC (ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize Die Version$^{\S}$} 
 & {\em \footnotesize tRP} 
 & {\em \footnotesize tRCD} \\

\midrule

%% MICRON
\cellcolor{white} & \module{B}{ 1}{} & 10-09 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 2}{} & 10-22 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\ 
\cellcolor{white} & \module{B}{ 3}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 4}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 5}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 6}{} & 11-26 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 7}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.1  & --   \\
\cellcolor{white} & \module{B}{ 8}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 479  & --   \\
\cellcolor{white} & \module{B}{ 9}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 1.9  & --   \\
\cellcolor{white} & \module{B}{10}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 4.3  & --   \\
\cellcolor{white} & \module{B}{11}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 161  & --   \\
\cellcolor{white} & \module{B}{12}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.3  & --   \\
\cellcolor{white} & \module{B}{13}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 16.0 & --   \\
\cellcolor{white} & \module{B}{14}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.6  & --   \\
\cellcolor{white} & \module{B}{15}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{16}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{17}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{18}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{19}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{20}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{21}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 4.3  & 11.4 \\
\cellcolor{white} & \module{B}{22}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 472  & --   \\
\cellcolor{white} & \module{B}{23}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 279  & --   \\
\cellcolor{white} & \module{B}{24}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 3276 & --   \\
\cellcolor{white} & \module{B}{25}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{26}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{27}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{28}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 78.3 & 8.2  \\
\cellcolor{white} & \module{B}{29}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 23.4 & 5.8  \\
\multirow{-32}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{B}{30}{} & 14-09 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\

\bottomrule

\end{tabular}

\begin{tabular}{lp{10cm}}

{$\,$} \\

{\footnotesize $\ast$ We report the manufacturing date in a year-week (yy-ww)
format. For example, 15-01 means that the DIMM was manufactured during} \\
{\hspace{0.1in}the first week of 2015.} \\ 

{$\,$} \\

{\footnotesize $\ddagger$ The maximum DRAM chip size supported by our testing
platform is 2Gb.} \\

{$\,$} \\

{\footnotesize $\S$ We report the DRAM die versions that are marked on the chip package.
Since the die version changes when the DRAM design changes,}\\
{\hspace{0.1in}we expect and observe that DIMMs with the same die version have similar
design-induced variation.} \\

{$\,$} \\

{\footnotesize $\star$ We report the {\em vulnerability ratio}, which we
define as the ratio of the number errors that occur the top 10\% of the most vulnerable and}\\
{\hspace{0.1in}least vulnerable rows, to show design-induced variation in timing parameters.}
\\

\end{tabular}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em B} (sorted by manufacturing date)} 
\label{tbl:vendor2}

\end{table*}


\newpage

\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Design-Induced Variation$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} 

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize tRC (ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize Die Version$^{\S}$} 
 & {\em \footnotesize tRP} 
 & {\em \footnotesize tRCD} \\

\midrule


%% SAMSUNG
\cellcolor{white} & \module{C}{ 1}{} & 08-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 2}{} & 09-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{E}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 3}{} & 10-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 4}{} & 11-16 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 5}{} & 11-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 6}{} & 11-25 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 7}{} & 11-37 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 2.6  \\
\cellcolor{white} & \module{C}{ 8}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 32.9 \\
\cellcolor{white} & \module{C}{ 9}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 42.3 \\
\cellcolor{white} & \module{C}{10}{} & 11-49 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{11}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 104  \\
\cellcolor{white} & \module{C}{12}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 117  \\
\cellcolor{white} & \module{C}{13}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 291  \\
\cellcolor{white} & \module{C}{14}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{15}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 97.0 \\
\cellcolor{white} & \module{C}{16}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 493  \\
\cellcolor{white} & \module{C}{17}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 61.8 \\
\cellcolor{white} & \module{C}{18}{} & 12-25 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.2  & 3.3  \\
\cellcolor{white} & \module{C}{19}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 473  & 3.1  \\
\cellcolor{white} & \module{C}{20}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 5.4  & 2.7  \\
\cellcolor{white} & \module{C}{21}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 3.5  & 3.0  \\
\cellcolor{white} & \module{C}{22}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 545  & 3.0  \\
\cellcolor{white} & \module{C}{23}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.7  & 3.0  \\
\cellcolor{white} & \module{C}{24}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 27.2 & 2.9  \\
\cellcolor{white} & \module{C}{25}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.3  \\
\cellcolor{white} & \module{C}{26}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 54.2 & 19.1 \\
\cellcolor{white} & \module{C}{27}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.1  \\
\cellcolor{white} & \module{C}{28}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 29.0 & 5.4  \\
\cellcolor{white} & \module{C}{29}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 120  & 6.7  \\
\cellcolor{white} & \module{C}{30}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 196  & 3.2  \\
\cellcolor{white} & \module{C}{31}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 599  & 8.5  \\
\cellcolor{white} & \module{C}{32}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 51.6 & --   \\
\cellcolor{white} & \module{C}{33}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.5  \\
\cellcolor{white} & \module{C}{34}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.6  \\
\cellcolor{white} & \module{C}{35}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.6  \\
\multirow{-38}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 36 DIMMs}
\cellcolor{white} & \module{C}{36}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.9  \\
\bottomrule

\end{tabular}

\begin{tabular}{lp{10cm}}

{$\,$} \\

{\footnotesize $\ast$ We report the manufacturing date in a year-week (yy-ww)
format. For example, 15-01 means that the DIMM was manufactured during} \\
{\hspace{0.1in}the first week of 2015.} \\ 

{$\,$} \\

{\footnotesize $\ddagger$ The maximum DRAM chip size supported by our testing
platform is 2Gb.} \\

{$\,$} \\

{\footnotesize $\S$ We report the DRAM die versions that are marked on the chip package.
Since the die version changes when the DRAM design changes,}\\
{\hspace{0.1in}we expect and observe that DIMMs with the same die version have similar
design-induced variation.} \\

{$\,$} \\

{\footnotesize $\star$ We report the {\em vulnerability ratio}, which we
define as the ratio of the number errors that occur the top 10\% of the most vulnerable and}\\
{\hspace{0.1in}least vulnerable rows, to show design-induced variation in timing parameters.}
\\

\end{tabular}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em C} (sorted by manufacturing date)} 
\label{tbl:vendor3}

\end{table*}


==> tbl/repo/modules_bak.tex <==

% \robustify\bfseries
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

%\sisetup{detect-weight=true, detect-inline-weight=math}
%\rowcolors{2}{lightgray}{white}
%\begin{tabular}{cl*{8}{c}*{3}{S[table-format=1.1e1]}S[table-format=2.1]}
%\begin{tabular}{cl*{8}{c}*{3}{}}
\begin{tabular}{ccccccccccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{3}{c}{\em \footnotesize \centering Victims-per-Module} &
                  {\em \footnotesize \centering $\mathit{RI}_{\mathit{th}}$}~{\em (ms)} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-14}

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize tRC(ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize DieVersion$^{\S}$} 
 & {\em \footnotesize Average} 
 & {\em \footnotesize Minimum} 
 & {\em \footnotesize Maximum} 
 & {\em \footnotesize Min} \\

\midrule

\cellcolor{white} & \module{A}{1}{} & 10-08 & 1066 & 50.625 & 0.5 & 4 & 1 & $\times$16 & $\mathcal{B}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{2}{} & 10-20 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{3\mhyphen 5}{} & 10-20 & 1066 & 50.625 & 0.5 & 4 & 1 & $\times$16 & $\mathcal{B}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{6\mhyphen 7}{} & 11-24 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 7.8e+01 & 5.2e+01 & 1.0e+02 & 21.3 \\
\cellcolor{white} & \module{A}{8\mhyphen 12}{} & 11-26 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.4e+02 & 5.4e+01 & 4.4e+02 & 16.4 \\
\cellcolor{white} & \module{A}{13\mhyphen 14}{} & 11-50 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.8e+01 & 1.7e+01 & 1.6e+02 & 26.2 \\
\cellcolor{white} & \module{A}{15\mhyphen 16}{} & 12-22 & 1600 & 50.625 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 9.5e+00 & 9 & 1.0e+01 & 34.4 \\
\cellcolor{white} & \module{A}{17\mhyphen 18}{} & 12-26 & 1600 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{M}$ & 1.2e+02 & 3.7e+01 & 2.0e+02 & 21.3 \\
\cellcolor{white} & \module{A}{19\mhyphen 30}{} & 12-40 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 8.6e+06 & 7.0e+06 & \bfseries 1.0e+07& \bfseries 8.2 \\
\cellcolor{white} & \module{A}{31\mhyphen 34}{} & 13-02 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & -- & 1.8e+06 & 1.0e+06 & 3.5e+06 & 11.5 \\
\cellcolor{white} & \module{A}{35\mhyphen 36}{} & 13-14 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & -- & 4.0e+01 & 1.9e+01 & 6.1e+01 & 21.3 \\
\cellcolor{white} & \module{A}{37\mhyphen 38}{} & 13-20 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 1.7e+06 & 1.4e+06 & 2.0e+06 & 9.8 \\
\cellcolor{white} & \module{A}{39\mhyphen 40}{} & 13-28 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 5.7e+04 & 5.4e+04 & 6.0e+04 & 16.4 \\
\cellcolor{white} & \module{A}{41}{} & 14-04 & 1600 & 49.125 & 2 & 8 & 2 & $\times$8 & -- & 2.7e+05 & 2.7e+05 & 2.7e+05 & 18.0 \\

\multirow{-15}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 43 Modules}
%\multirow{-15}{5em}{\centering {\large\a} \\ {\tiny \quad \\} \centering Total of \\ \centering 43 Modules}

\cellcolor{white} & \module{A}{42\mhyphen 43}{} & 14-04 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 0.5 & 0 & 1 & 62.3 \global\rownum=10\\
\cmidrule(lr){1-14}
\cellcolor{white} & \module{B}{1}{} & 08-49 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{D}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{2}{} & 09-49 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{E}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{3}{} & 10-19 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{4}{} & 10-31 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{5}{} & 11-13 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{6}{} & 11-16 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{7}{} & 11-19 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{8}{} & 11-25 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{9}{} & 11-37 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 1.9e+06 & 1.9e+06 & 1.9e+06 & 11.5 \\
\cellcolor{white} & \module{B}{10\mhyphen 12}{} & 11-46 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 2.2e+06 & 1.5e+06 & \bfseries 2.7e+06& 11.5 \\
\cellcolor{white} & \module{B}{13}{} & 11-49 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{14}{} & 12-01 & 1866 & 47.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 9.1e+05 & 9.1e+05 & 9.1e+05 & \bfseries 9.8 \\
\cellcolor{white} & \module{B}{15\mhyphen 31}{} & 12-10 & 1866 & 47.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 9.8e+05 & 7.8e+05 & 1.2e+06 & 11.5 \\
\cellcolor{white} & \module{B}{32}{} & 12-25 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 7.4e+05 & 7.4e+05 & 7.4e+05 & 11.5 \\
\cellcolor{white} & \module{B}{33\mhyphen 42}{} & 12-28 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 5.2e+05 & 1.9e+05 & 7.3e+05 & 11.5 \\
\cellcolor{white} & \module{B}{43\mhyphen 47}{} & 12-31 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 4.0e+05 & 2.9e+05 & 5.5e+05 & 13.1 \\
\cellcolor{white} & \module{B}{48\mhyphen 51}{} & 13-19 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 1.1e+05 & 7.4e+04 & 1.4e+05 & 14.7 \\
\cellcolor{white} & \module{B}{52\mhyphen 53}{} & 13-40 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 2.6e+04 & 2.3e+04 & 2.9e+04 & 21.3 \\
\multirow{-19}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 54 Modules}
\cellcolor{white} & \module{B}{54}{} & 14-07 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 7.5e+03 & 7.5e+03 & 7.5e+03 & 26.2 \global\rownum=11\\
\cmidrule(lr){1-14}
\cellcolor{white} & \module{C}{1}{} & 10-18 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{2}{} & 10-20 & 1066 & 50.625 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{3}{} & 10-22 & 1066 & 50.625 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{4\mhyphen 5}{} & 10-26 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 8.9e+02 & 6.0e+02 & 1.2e+03 & 29.5 \\
\cellcolor{white} & \module{C}{6}{} & 10-43 & 1333 & 49.125 & 1 & 8 & 1 & $\times$8 & $\mathcal{T}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{7}{} & 10-51 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 4.0e+02 & 4.0e+02 & 4.0e+02 & 29.5 \\
\cellcolor{white} & \module{C}{8}{} & 11-12 & 1333 & 46.25 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 6.9e+02 & 6.9e+02 & 6.9e+02 & 21.3 \\
\cellcolor{white} & \module{C}{9}{} & 11-19 & 1333 & 46.25 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 9.2e+02 & 9.2e+02 & 9.2e+02 & 27.9 \\
\cellcolor{white} & \module{C}{10}{} & 11-31 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 3 & 3 & 3 & 39.3 \\
\cellcolor{white} & \module{C}{11}{} & 11-42 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 1.6e+02 & 1.6e+02 & 1.6e+02 & 39.3 \\
\cellcolor{white} & \module{C}{12}{} & 11-48 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 7.1e+04 & 7.1e+04 & 7.1e+04 & 19.7 \\
\cellcolor{white} & \module{C}{13}{} & 12-08 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.9e+04 & 3.9e+04 & 3.9e+04 & 21.3 \\
\cellcolor{white} & \module{C}{14\mhyphen 15}{} & 12-12 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.7e+04 & 2.1e+04 & 5.4e+04 & 21.3 \\
\cellcolor{white} & \module{C}{16\mhyphen 18}{} & 12-20 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.5e+03 & 1.2e+03 & 7.0e+03 & 27.9 \\
\cellcolor{white} & \module{C}{19}{} & 12-23 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 1.4e+05 & 1.4e+05 & 1.4e+05 & 18.0 \\
\cellcolor{white} & \module{C}{20}{} & 12-24 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 6.5e+04 & 6.5e+04 & 6.5e+04 & 21.3 \\
\cellcolor{white} & \module{C}{21}{} & 12-26 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.3e+04 & 2.3e+04 & 2.3e+04 & 24.6 \\
\cellcolor{white} & \module{C}{22}{} & 12-32 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 1.7e+04 & 1.7e+04 & 1.7e+04 & 22.9 \\
\cellcolor{white} & \module{C}{23\mhyphen 24}{} & 12-37 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.3e+04 & 1.1e+04 & 3.4e+04 & 18.0 \\
\cellcolor{white} & \module{C}{25\mhyphen 30}{} & 12-41 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.0e+04 & 1.1e+04 & 3.2e+04 & 19.7 \\
\cellcolor{white} & \module{C}{31}{} & 13-11 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.3e+05 & 3.3e+05 & \bfseries 3.3e+05& \bfseries 14.7 \\
\multirow{-22}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 32 Modules}
\cellcolor{white} & \module{C}{32}{} & 13-35 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.7e+04 & 3.7e+04 & 3.7e+04 & 21.3 \global\rownum=11\\

\bottomrule

% \rowcolor{white} \multicolumn{14}{r}{$\,$} \\
%
% \rowcolor{white} \multicolumn{14}{r}{\footnotesize $\ast$ We report the
% manufacture date marked on the chip packages, which is more accurate
% than other dates that can be gleaned from a module.} \\
%
% \rowcolor{white} \multicolumn{14}{r}{\footnotesize $\dagger$ We report
% timing constraints stored in the module's on-board ROM~\cite{jedec-spd},
% which is read by the system BIOS to calibrate the memory controller.} \\
%
% \rowcolor{white} \multicolumn{14}{r}{\footnotesize $\ddagger$ The
% maximum DRAM chip size supported by our testing platform is 2Gb.} \\
%
% \rowcolor{white} \multicolumn{14}{r}{\footnotesize $\S$ We report DRAM
% die versions marked on the chip packages, which typically progress in
% the following manner: $\mathcal{M} \shortrightarrow \mathcal{A}
% \shortrightarrow \mathcal{B} \shortrightarrow \mathcal{C}
% \shortrightarrow \cdots$.} \\

\end{tabular}

\caption{Sample population of 129 DDR3 DRAM modules,
categorized by manufacturer and sorted by manufacture date} 

\label{tab:modules}

\end{table*}


==> tbl/repo/modules_bak2.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table}[h]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Design-Induced Variation} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} 

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize tRC(ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize DieVersion$^{\S}$} 
 & {\em \footnotesize tRP} 
 & {\em \footnotesize tRCD} \\

\midrule

%% MICRON
\cellcolor{white} & \module{A}{ 1}{} & 10-09 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{A}{ 2}{} & 10-22 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\ 
\cellcolor{white} & \module{A}{ 3}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{A}{ 5}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{A}{ 6}{} & 11-26 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & --   & --   \\
\cellcolor{white} & \module{A}{ 7}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.1  & --   \\
\cellcolor{white} & \module{A}{ 8}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 479  & --   \\
\cellcolor{white} & \module{A}{ 9}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 1.9  & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 4.3  & --   \\
\cellcolor{white} & \module{A}{11}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 161  & --   \\
\cellcolor{white} & \module{A}{12}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.3  & --   \\
\cellcolor{white} & \module{A}{13}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 16.0 & --   \\
\cellcolor{white} & \module{A}{14}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.6  & --   \\
\cellcolor{white} & \module{A}{15}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{A}{16}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{A}{17}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{A}{18}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{A}{19}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{A}{20}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{A}{21}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 4.3  & 11.4 \\
\cellcolor{white} & \module{A}{22}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 472  & --   \\
\cellcolor{white} & \module{A}{23}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 279  & --   \\
\cellcolor{white} & \module{A}{24}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 3276 & --   \\
\cellcolor{white} & \module{A}{25}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{A}{26}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{A}{27}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{A}{28}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 78.3 & 8.2  \\
\cellcolor{white} & \module{A}{29}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 23.4 & 5.8  \\
\multirow{-28}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 14-09 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\

\cmidrule(lr){1-12}
%% SAMSUNG
\cellcolor{white} & \module{B}{ 1}{} & 08-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 2}{} & 09-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{E}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 3}{} & 10-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 6}{} & 11-16 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 7}{} & 11-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 8}{} & 11-25 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{ 9}{} & 11-37 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 2.6  \\
\cellcolor{white} & \module{B}{10}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 32.9 \\
\cellcolor{white} & \module{B}{12}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 42.3 \\
\cellcolor{white} & \module{B}{13}{} & 11-49 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{16}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 104  \\
\cellcolor{white} & \module{B}{18}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 117  \\
\cellcolor{white} & \module{B}{19}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 291  \\
\cellcolor{white} & \module{B}{20}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{B}{21}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 97.0 \\
\cellcolor{white} & \module{B}{22}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 493  \\
\cellcolor{white} & \module{B}{23}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 61.8 \\
\cellcolor{white} & \module{B}{32}{} & 12-25 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.2  & 3.3  \\
\cellcolor{white} & \module{B}{33}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 473  & 3.1  \\
\cellcolor{white} & \module{B}{34}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 5.4  & 2.7  \\
\cellcolor{white} & \module{B}{35}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 3.5  & 3.0  \\
\cellcolor{white} & \module{B}{36}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 545  & 3.0  \\
\cellcolor{white} & \module{B}{37}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.7  & 3.0  \\
\cellcolor{white} & \module{B}{38}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 27.2 & 2.9  \\
\cellcolor{white} & \module{B}{39}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.3  \\
\cellcolor{white} & \module{B}{40}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 54.2 & 19.1 \\
\cellcolor{white} & \module{B}{42}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.1  \\
\cellcolor{white} & \module{B}{43}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 29.0 & 5.4  \\
\cellcolor{white} & \module{B}{44}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 120  & 6.7  \\
\cellcolor{white} & \module{B}{45}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 196  & 3.2  \\
\cellcolor{white} & \module{B}{46}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 599  & 8.5  \\
\cellcolor{white} & \module{B}{47}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 51.6 & --   \\
\cellcolor{white} & \module{B}{48}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.5  \\
\cellcolor{white} & \module{B}{49}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.6  \\
\cellcolor{white} & \module{B}{50}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.6  \\
\multirow{-34}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 36 DIMMs}
\cellcolor{white} & \module{B}{51}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.9  \\


\cmidrule(lr){1-12}
%% HYNIX
\cellcolor{white} & \module{C}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{C}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{C}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{C}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{C}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{C}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{C}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{C}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{C}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\cellcolor{white} & \module{C}{11}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{12}{} & 11-31 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 4.3  & --	  \\
\cellcolor{white} & \module{C}{13}{} & 11-42 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 4.9  & 93.7 \\
\cellcolor{white} & \module{C}{14}{} & 12-08 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 96.7 & 28.6 \\
\cellcolor{white} & \module{C}{15}{} & 12-12 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 3.9  & 45.2 \\
\cellcolor{white} & \module{C}{16}{} & 12-12 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 103  & 373  \\
\cellcolor{white} & \module{C}{17}{} & 12-20 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 31.4 & 178  \\
\cellcolor{white} & \module{C}{18}{} & 12-20 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{19}{} & 12-24 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 37.1 & 21.3 \\
\cellcolor{white} & \module{C}{20}{} & 12-26 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 26.7 & 26.9 \\
\cellcolor{white} & \module{C}{21}{} & 12-32 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 61.3 & 160  \\
\cellcolor{white} & \module{C}{22}{} & 12-37 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 9.9  & 44.3 \\
\cellcolor{white} & \module{C}{23}{} & 12-37 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 161  & 37.1 \\
\cellcolor{white} & \module{C}{24}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 54.4 & 196  \\
\cellcolor{white} & \module{C}{25}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 24.1 & 1034 \\
\cellcolor{white} & \module{C}{26}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 208  & 55.8 \\
\cellcolor{white} & \module{C}{27}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 88.3 & 20.8 \\
\cellcolor{white} & \module{C}{28}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 51.6 & 122  \\
\cellcolor{white} & \module{C}{29}{} & 12-41 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 31.8 & 100  \\
\multirow{-28}{5em}{\centering {\large} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{C}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\


\bottomrule

\end{tabular}

\caption{Sample population of 96 DDR3 DIMMs, categorized by manufacturer and sorted by manufacture date} 

\end{table}


==> tbl/repo/modules_yg.tex <==

\robustify\bfseries
\definecolor{lightgray}{gray}{0.95}

%\newcolumntype{w}{>{\columncolor{white}}c}

% -- begin:
%\afterpage{


\begin{table*}[t]
%\vskip -5pt

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
%\scriptsize
\sisetup{detect-weight=true, detect-inline-weight=math}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{cl*{8}{c}*{3}{S[table-format=1.1e1]}S[table-format=2.1]}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Manufacturer} & 
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} & 
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{3}{c}{\em \footnotesize \centering Victims-per-Module} &
                  {\em \footnotesize \centering $\mathit{RI}_{\mathit{th}}$}~{\em (ms)} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-14}

%{\em $\mathit{RI}_{th}$ (ms)}

 & 
 & {\em \footnotesize (yy-ww)} 
 & {\em \footnotesize Freq~(MT/s)} 
 & {\em \footnotesize \trc(ns)} 
 & {\em \footnotesize Size (GB)} 
 & {\em \footnotesize Chips} 
 & {\em \footnotesize Size (Gb)$^{\ddagger}$} 
 & {\em \footnotesize Pins} 
 & {\em \footnotesize DieVersion$^{\S}$} 
 & {\em \footnotesize Average} 
 & {\em \footnotesize Minimum} 
 & {\em \footnotesize Maximum} 
 & {\em \footnotesize Min} \\


\midrule

\cellcolor{white} & \module{A}{1}{} & 10-08 & 1066 & 50.625 & 0.5 & 4 & 1 & $\times$16 & $\mathcal{B}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{2}{} & 10-20 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{3\mhyphen 5}{} & 10-20 & 1066 & 50.625 & 0.5 & 4 & 1 & $\times$16 & $\mathcal{B}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{A}{6\mhyphen 7}{} & 11-24 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 7.8e+01 & 5.2e+01 & 1.0e+02 & 21.3 \\
\cellcolor{white} & \module{A}{8\mhyphen 12}{} & 11-26 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.4e+02 & 5.4e+01 & 4.4e+02 & 16.4 \\
\cellcolor{white} & \module{A}{13\mhyphen 14}{} & 11-50 & 1066 & 49.125 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.8e+01 & 1.7e+01 & 1.6e+02 & 26.2 \\
\cellcolor{white} & \module{A}{15\mhyphen 16}{} & 12-22 & 1600 & 50.625 & 1 & 4 & 2 & $\times$16 & $\mathcal{D}$ & 9.5e+00 & 9 & 1.0e+01 & 34.4 \\
\cellcolor{white} & \module{A}{17\mhyphen 18}{} & 12-26 & 1600 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{M}$ & 1.2e+02 & 3.7e+01 & 2.0e+02 & 21.3 \\
\cellcolor{white} & \module{A}{19\mhyphen 30}{} & 12-40 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 8.6e+06 & 7.0e+06 & \bfseries 1.0e+07& \bfseries 8.2 \\
\cellcolor{white} & \module{A}{31\mhyphen 34}{} & 13-02 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & -- & 1.8e+06 & 1.0e+06 & 3.5e+06 & 11.5 \\
\cellcolor{white} & \module{A}{35\mhyphen 36}{} & 13-14 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & -- & 4.0e+01 & 1.9e+01 & 6.1e+01 & 21.3 \\
\cellcolor{white} & \module{A}{37\mhyphen 38}{} & 13-20 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 1.7e+06 & 1.4e+06 & 2.0e+06 & 9.8 \\
\cellcolor{white} & \module{A}{39\mhyphen 40}{} & 13-28 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 5.7e+04 & 5.4e+04 & 6.0e+04 & 16.4 \\
\cellcolor{white} & \module{A}{41}{} & 14-04 & 1600 & 49.125 & 2 & 8 & 2 & $\times$8 & -- & 2.7e+05 & 2.7e+05 & 2.7e+05 & 18.0 \\
\multirow{-15}{5em}{\centering {\large\a} \\ {\tiny \quad \\} \centering Total of \\ \centering 43 Modules}
\cellcolor{white} & \module{A}{42\mhyphen 43}{} & 14-04 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{K}$ & 0.5 & 0 & 1 & 62.3 \global\rownum=10\\
\cmidrule(lr){1-14}
\cellcolor{white} & \module{B}{1}{} & 08-49 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{D}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{2}{} & 09-49 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{E}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{3}{} & 10-19 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{4}{} & 10-31 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{5}{} & 11-13 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{6}{} & 11-16 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{7}{} & 11-19 & 1066 & 50.625 & 1 & 8 & 1 & $\times$8 & $\mathcal{F}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{8}{} & 11-25 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{9}{} & 11-37 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 1.9e+06 & 1.9e+06 & 1.9e+06 & 11.5 \\
\cellcolor{white} & \module{B}{10\mhyphen 12}{} & 11-46 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 2.2e+06 & 1.5e+06 & \bfseries 2.7e+06& 11.5 \\
\cellcolor{white} & \module{B}{13}{} & 11-49 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{B}{14}{} & 12-01 & 1866 & 47.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 9.1e+05 & 9.1e+05 & 9.1e+05 & \bfseries 9.8 \\
\cellcolor{white} & \module{B}{15\mhyphen 31}{} & 12-10 & 1866 & 47.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 9.8e+05 & 7.8e+05 & 1.2e+06 & 11.5 \\
\cellcolor{white} & \module{B}{32}{} & 12-25 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 7.4e+05 & 7.4e+05 & 7.4e+05 & 11.5 \\
\cellcolor{white} & \module{B}{33\mhyphen 42}{} & 12-28 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 5.2e+05 & 1.9e+05 & 7.3e+05 & 11.5 \\
\cellcolor{white} & \module{B}{43\mhyphen 47}{} & 12-31 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 4.0e+05 & 2.9e+05 & 5.5e+05 & 13.1 \\
\cellcolor{white} & \module{B}{48\mhyphen 51}{} & 13-19 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 1.1e+05 & 7.4e+04 & 1.4e+05 & 14.7 \\
\cellcolor{white} & \module{B}{52\mhyphen 53}{} & 13-40 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 2.6e+04 & 2.3e+04 & 2.9e+04 & 21.3 \\
\multirow{-19}{5em}{\centering {\large\b} \\ {\tiny \quad \\} \centering Total of \\ \centering 54 Modules}
\cellcolor{white} & \module{B}{54}{} & 14-07 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{D}$ & 7.5e+03 & 7.5e+03 & 7.5e+03 & 26.2 \global\rownum=11\\
\cmidrule(lr){1-14}
\cellcolor{white} & \module{C}{1}{} & 10-18 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{2}{} & 10-20 & 1066 & 50.625 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{3}{} & 10-22 & 1066 & 50.625 & 2 & 8 & 2 & $\times$8 & $\mathcal{A}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{4\mhyphen 5}{} & 10-26 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 8.9e+02 & 6.0e+02 & 1.2e+03 & 29.5 \\
\cellcolor{white} & \module{C}{6}{} & 10-43 & 1333 & 49.125 & 1 & 8 & 1 & $\times$8 & $\mathcal{T}$ & 0 & 0 & 0 & \text{--} \\
\cellcolor{white} & \module{C}{7}{} & 10-51 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 4.0e+02 & 4.0e+02 & 4.0e+02 & 29.5 \\
\cellcolor{white} & \module{C}{8}{} & 11-12 & 1333 & 46.25 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 6.9e+02 & 6.9e+02 & 6.9e+02 & 21.3 \\
\cellcolor{white} & \module{C}{9}{} & 11-19 & 1333 & 46.25 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 9.2e+02 & 9.2e+02 & 9.2e+02 & 27.9 \\
\cellcolor{white} & \module{C}{10}{} & 11-31 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 3 & 3 & 3 & 39.3 \\
\cellcolor{white} & \module{C}{11}{} & 11-42 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{B}$ & 1.6e+02 & 1.6e+02 & 1.6e+02 & 39.3 \\
\cellcolor{white} & \module{C}{12}{} & 11-48 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 7.1e+04 & 7.1e+04 & 7.1e+04 & 19.7 \\
\cellcolor{white} & \module{C}{13}{} & 12-08 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.9e+04 & 3.9e+04 & 3.9e+04 & 21.3 \\
\cellcolor{white} & \module{C}{14\mhyphen 15}{} & 12-12 & 1333 & 49.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.7e+04 & 2.1e+04 & 5.4e+04 & 21.3 \\
\cellcolor{white} & \module{C}{16\mhyphen 18}{} & 12-20 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.5e+03 & 1.2e+03 & 7.0e+03 & 27.9 \\
\cellcolor{white} & \module{C}{19}{} & 12-23 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{E}$ & 1.4e+05 & 1.4e+05 & 1.4e+05 & 18.0 \\
\cellcolor{white} & \module{C}{20}{} & 12-24 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 6.5e+04 & 6.5e+04 & 6.5e+04 & 21.3 \\
\cellcolor{white} & \module{C}{21}{} & 12-26 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.3e+04 & 2.3e+04 & 2.3e+04 & 24.6 \\
\cellcolor{white} & \module{C}{22}{} & 12-32 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 1.7e+04 & 1.7e+04 & 1.7e+04 & 22.9 \\
\cellcolor{white} & \module{C}{23\mhyphen 24}{} & 12-37 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.3e+04 & 1.1e+04 & 3.4e+04 & 18.0 \\
\cellcolor{white} & \module{C}{25\mhyphen 30}{} & 12-41 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 2.0e+04 & 1.1e+04 & 3.2e+04 & 19.7 \\
\cellcolor{white} & \module{C}{31}{} & 13-11 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.3e+05 & 3.3e+05 & \bfseries 3.3e+05& \bfseries 14.7 \\
\multirow{-22}{5em}{\centering {\large\c} \\ {\tiny \quad \\} \centering Total of \\ \centering 32 Modules}
\cellcolor{white} & \module{C}{32}{} & 13-35 & 1600 & 48.125 & 2 & 8 & 2 & $\times$8 & $\mathcal{C}$ & 3.7e+04 & 3.7e+04 & 3.7e+04 & 21.3 \global\rownum=11\\



\bottomrule

\rowcolor{white} \multicolumn{14}{r}{$\,$} \\

\rowcolor{white} \multicolumn{14}{r}{\footnotesize $\ast$ We report the
manufacture date marked on the chip packages, which is more accurate
than other dates that can be gleaned from a module.} \\

%. This is a more accurate than using other
%dates that can be gleaned from a module (manufacturer's label or on-board
%ROM~\cite{jedec-spd}

%As many as three different dates can be gleaned from a module:
%manufacturer's label, on-board ROM~\cite{jedec-spd}, and chip-package
%markings. As many as three different manufacture dates can be gleaned
%from a module.

\rowcolor{white} \multicolumn{14}{r}{\footnotesize $\dagger$ We report
timing constraints stored in the module's on-board ROM~\cite{jedec-spd},
which is read by the system BIOS to calibrate the memory controller.} \\

\rowcolor{white} \multicolumn{14}{r}{\footnotesize $\ddagger$ The
maximum DRAM chip size supported by our testing platform is 2Gb.} \\

\rowcolor{white} \multicolumn{14}{r}{\footnotesize $\S$ We report DRAM
die versions marked on the chip packages, which typically progress in
the following manner: $\mathcal{M} \shortrightarrow \mathcal{A}
\shortrightarrow \mathcal{B} \shortrightarrow \mathcal{C}
\shortrightarrow \cdots$.} \\

\end{tabular}

%\vspace{-1ex}
%\vspace{1ex}

%\footnotesize 
\caption{Sample population of 129 DDR3 DRAM modules,
categorized by manufacturer and sorted by manufacture date} 

%. Each row in the table corresponds to a {\em family} of modules. For
%each family, three right columns list the average/minimum/maximum
%numbers of disturbance errors induced among the modules of that family
%(Section~\ref{subsec:widespread}). The rightmost column lists the
%refresh interval that is needed to eliminate all errors for the modules
%of that family (Section~\ref{subsec:access-pattern}).

\label{tab:modules}

\end{table*}

% -- end:
%}


